Consistent dust and gas models for protoplanetary disks III. Models for selected objects from the FP7 DIANA project

The European FP7 project DIANA has performed a coherent analysis of a large set of observations from protoplanetary disks by means of thermo-chemical disk models. The collected data include extinction-corrected stellar UV and X-ray input spectra (as seen by the disk), photometric fluxes, low and high resolution spectra, interferometric data, emission line fluxes, line velocity profiles and line maps. We define and apply a standardized modelling procedure to simultaneously fit all these data by state-of-the-art modelling codes (ProDiMo, MCFOST, MCMax) which solve the continuum and line radiative transfer, disk chemistry, and the heating & cooling balance for both the gas and the dust. We allow for up to two radial disk zones to obtain our best-fitting models that have about 20 free parameters. This approach is novel and unique in its completeness and level of consistency. In this paper, we present the results from pure SED fitting for 27 objects and from the all inclusive DIANA-standard models for 14 objects. We fit most infrared to millimeter emission line fluxes within a factor better than 3, simultaneously with SED, PAH features and radial brightness profiles extracted from images at various wavelengths. Our analysis shows a number of Herbig Ae and T Tauri stars with very cold and massive outer disks which are situated at least partly in the shadow of a tall and gas-rich inner disk. The disk masses derived are often in excess to previously published values, since these disks are partially optically thick even at millimeter wavelength and so cold that they emit less than in the Rayleigh-Jeans limit. Some line observations cannot be reproduced by the models, probably caused by foreground cloud absorption or object variability. Our data collection, the fitted physical disk parameters as well as the full model output are available at an online database (http://www.univie.ac.at/diana).

==> DIANAmodels/ABAur.tex <==
\centering
\begin{tabular}{rr}
\hline
DIANA standard fit model properties &  \\
\hline
minimum dust temperature [K] & 20.95 \\
maximum dust temperature [K] & 1830.20 \\
mass-mean dust temperature [K] & 36.05 \\
minimum  gas temperature [K] & 25.52 \\
maximum  gas temperature [K] & 23349.23 \\
mass-mean  gas temperature [K] & 54.12 \\
mm-opacity-slope (0.85-1.3)mm & 1.71 \\
cm-opacity-slope (5-10)mm & 1.79 \\
mm-SED-slope (0.85-1.3)mm & 3.51 \\
cm-SED-slope (5-10)mm & 3.57 \\
10$\mathrm{\mu m}$ silicate emission amplitude & 1.62 \\
naked star luminosity [$L_\odot$] & 41.29 \\
bolometric luminosity [$L_\odot$] & 70.36 \\
near IR excess ($\lambda=$2.01-6.82$\mathrm{\mu m}$)
 [$L_\odot$] & 8.56 \\
mid IR excess ($\lambda=$6.82-29.3$\mathrm{\mu m}$)
 [$L_\odot$] & 5.12 \\
far IR excess ($\lambda=$29.3-999.$\mathrm{\mu m}$)
 [$L_\odot$] & 4.74 \\
\hline
\end{tabular}


\vspace{0.5cm}
\centering\begin{tabular}{lrccccr}
\hline\\[-2mm]
  & & \multicolumn{2}{c}{line flux $[\mathrm{W\,m^{-2}}$]} & \multicolumn{2}{c}{FWHM[$\mathrm{km\,s^{-1}}$]} &  \\
species & $\lambda\,$[$\mathrm{\mu m}]$ & observed & model & observed & model & size[AU] \\
\hline
$\mathrm{OI}$ & 63.183 & 8.51$\pm$0.21(-16) & 2.59(-15) &  & 4.21 & 386.22 \\
$\mathrm{OI}$ & 145.525 & 4.46$\pm$1.47(-17) & 1.79(-16) &  & 3.89 & 319.60 \\
$\mathrm{OI}$ & 0.630 & 9.73$\pm$3.00(-16) & 1.69(-16) & 20.00$\pm$2.00 & 5.68 & 98.91 \\
$\mathrm{CII}$ & 157.740 & 5.10$\pm$0.83(-17) & 8.14(-17) &  & 2.65 & 615.63 \\
$\mathrm{C}$ & 370.415 & 5.60$\pm$2.80(-18) & 1.51(-17) &  & 2.84 & 536.63 \\
$\mathrm{HCO^+}$ & 3361.334 & 1.40$\pm$0.20(-21) & 1.08(-21) & 4.00$\pm$0.50 & 3.29 & 338.91 \\
$\mathrm{HCO^+}$ & 1120.478 & 4.80$\pm$1.00(-20) & 9.18(-20) & 2.50$\pm$0.50 & 3.37 & 384.46 \\
$\mathrm{CO}$ & 866.963 & 1.03$\pm$0.20(-18) & 2.67(-18) & 3.00$\pm$0.50 & 3.08 & 577.20 \\
$\mathrm{CO}$ & 1300.403 & 1.20$\pm$0.20(-19) & 7.49(-19) & 3.50$\pm$0.50 & 3.07 & 484.24 \\
$\mathrm{^{13}CO}$ & 1360.227 & 2.68$\pm$0.20(-19) & 2.13(-19) & 2.50$\pm$0.50 & 3.06 & 422.15 \\
$\mathrm{C^{18}O}$ & 1365.430 & 3.90$\pm$0.80(-20) & 8.52(-20) & 2.50$\pm$0.50 & 3.24 & 387.66 \\
$\mathrm{C^{17}O}$ & 1334.098 & 1.96$\pm$0.20(-20) & 3.65(-20) & 2.50$\pm$0.50 & 3.31 & 371.83 \\
$\mathrm{CN}$ & 1321.390 & 3.18$\pm$0.30(-21) & 8.49(-20) & 2.50$\pm$0.50 & 2.47 & 563.20 \\
$\mathrm{o\!-\!H_2CO}$ & 1419.394 & 2.61$\pm$0.30(-21) & 2.92(-21) & 2.50$\pm$0.50 & 3.14 & 415.07 \\
$\mathrm{o\!-\!H_2CO}$ & 1328.291 & 9.03$\pm$0.90(-21) & 3.62(-21) & 2.50$\pm$0.50 & 3.14 & 411.27 \\
$\mathrm{HCN}$ & 1127.520 & 1.10$\pm$0.20(-20) & 1.32(-19) & 2.50$\pm$0.50 & 2.63 & 486.51 \\
$\mathrm{CS}$ & 2039.834 & 1.80$\pm$0.40(-21) & 1.84(-21) & 2.50$\pm$0.50 & 2.74 & 515.93 \\
$\mathrm{SO}$ & 1454.060 & 1.40$\pm$0.30(-21) & 1.36(-21) & 2.50$\pm$0.50 & 3.64 & 293.61 \\
$\mathrm{SO}$ & 1363.006 & 1.90$\pm$0.40(-21) & 2.91(-21) & 2.50$\pm$0.50 & 3.64 & 300.28 \\
$\mathrm{CO}$ & 371.650 & 3.49$\pm$0.28(-17) & 2.96(-17) &  & 3.13 & 483.93 \\
$\mathrm{CO}$ & 325.225 & 4.30$\pm$0.36(-17) & 4.04(-17) &  & 3.16 & 472.62 \\
$\mathrm{CO}$ & 289.120 & 4.30$\pm$0.43(-17) & 5.18(-17) &  & 3.21 & 458.54 \\
$\mathrm{CO}$ & 260.239 & 4.11$\pm$0.40(-17) & 6.28(-17) &  & 3.24 & 441.51 \\
$\mathrm{CO}$ & 236.613 & 4.86$\pm$0.45(-17) & 7.24(-17) &  & 3.31 & 419.95 \\
$\mathrm{CO}$ & 216.927 & 3.83$\pm$0.38(-17) & 7.88(-17) &  & 3.45 & 389.17 \\
$\mathrm{CO}$ & 200.272 & 4.39$\pm$0.47(-17) & 8.17(-17) &  & 3.70 & 341.01 \\
$\mathrm{^{13}CO}$ & 388.743 & 3.80$\pm$2.50(-18) & 9.52(-18) &  & 3.16 & 416.92 \\
$\mathrm{^{13}CO}$ & 302.414 & 7.10$\pm$4.00(-18) & 1.38(-17) &  & 3.44 & 384.50 \\
$\mathrm{CO}$ & 72.842 & $<$3.78(-17) & 9.91(-19) &  & 5.68 & 97.53 \\
$\mathrm{CO}$ & 79.359 & $<$3.36(-17) & 2.90(-18) &  & 7.35 & 95.07 \\
$\mathrm{CO}$ & 90.162 & 3.10$\pm$0.43(-17) & 1.82(-17) &  & 7.49 & 78.44 \\
$\mathrm{CO}$ & 108.762 & $<$4.50(-17) & 7.54(-17) &  & 6.88 & 79.95 \\
$\mathrm{CO}$ & 113.457 & 5.89$\pm$1.24(-17) & 8.22(-17) &  & 6.82 & 81.15 \\
$\mathrm{CO}$ & 118.580 & $<$4.59(-17) & 8.51(-17) &  & 6.76 & 82.85 \\
$\mathrm{CO}$ & 124.193 & $<$3.51(-17) & 8.49(-17) &  & 6.76 & 86.30 \\
$\mathrm{CO}$ & 130.368 & 3.92$\pm$0.93(-17) & 8.33(-17) &  & 6.76 & 106.20 \\
$\mathrm{CO}$ & 137.196 & $<$2.91(-17) & 8.15(-17) &  & 6.65 & 128.96 \\
$\mathrm{CO}$ & 144.784 & 2.66$\pm$0.88(-17) & 8.09(-17) &  & 6.41 & 150.44 \\
$\mathrm{CO}$ & 153.266 & 4.07$\pm$1.44(-17) & 8.14(-17) &  & 5.83 & 173.86 \\
$\mathrm{CO}$ & 162.811 & $<$2.70(-17) & 8.20(-17) &  & 4.90 & 200.41 \\
$\mathrm{CO}$ & 173.631 & 6.40$\pm$1.61(-17) & 8.23(-17) &  & 4.44 & 234.09 \\
$\mathrm{CO}$ & 185.999 & $<$3.03(-17) & 8.24(-17) &  & 4.03 & 280.81 \\
\hline
\end{tabular}
\end{table}

\newpage
\addtocounter{table}{-1}

\begin{table}
\caption{(continued)}
\vspace{0.5cm}
\centering\begin{tabular}{lrccccr}
\hline\\[-2mm]
  & & \multicolumn{2}{c}{line flux $[\mathrm{W\,m^{-2}}$]} & \multicolumn{2}{c}{FWHM[$\mathrm{km\,s^{-1}}$]} &  \\
species & $\lambda\,$[$\mathrm{\mu m}]$ & observed & model & observed & model & size[AU] \\
\hline
$\mathrm{CO}$ & 4.633 & 1.36$\pm$0.25(-16) & 1.13(-16) & 23.10$\pm$2.00 & 11.26 & 92.08 \\
$\mathrm{CO}$ & 4.657 & 8.80$\pm$0.50(-17) & 7.59(-17) & 24.20$\pm$2.00 & 11.18 & 92.32 \\
$\mathrm{CO}$ & 4.674 & 8.10$\pm$0.50(-17) & 7.38(-17) & 22.80$\pm$2.00 & 11.26 & 92.32 \\
$\mathrm{CO}$ & 4.682 & 1.04$\pm$0.25(-16) & 9.35(-17) & 21.00$\pm$2.00 & 10.97 & 92.24 \\
$\mathrm{CO}$ & 4.699 & 1.37$\pm$0.25(-16) & 1.22(-16) & 20.80$\pm$2.00 & 10.68 & 92.25 \\
$\mathrm{CO}$ & 4.735 & 1.43$\pm$0.25(-16) & 1.31(-16) & 20.80$\pm$2.00 & 11.40 & 92.28 \\
$\mathrm{CO}$ & 4.773 & 1.45$\pm$0.25(-16) & 1.12(-16) & 20.90$\pm$2.00 & 37.10 & 92.10 \\
$\mathrm{CO}$ & 4.920 & 1.04$\pm$0.25(-16) & 8.54(-17) & 27.10$\pm$2.00 & 64.47 & 1.28 \\
$\mathrm{CO}$ & 4.966 & 7.60$\pm$0.50(-17) & 7.78(-17) & 25.60$\pm$2.00 & 65.62 & 1.10 \\
$\mathrm{CO}$ & 5.066 & 3.10$\pm$0.50(-17) & 6.18(-17) & 26.40$\pm$2.00 & 67.43 & 0.77 \\
$\mathrm{^{13}CO}$ & 4.643 & 1.40$\pm$0.30(-17) & 8.63(-18) & 20.20$\pm$2.00 & 41.95 & 0.48 \\
$\mathrm{^{13}CO}$ & 4.692 & 1.40$\pm$0.30(-17) & 7.11(-18) & 17.60$\pm$2.00 & 14.73 & 95.58 \\
$\mathrm{^{13}CO}$ & 4.738 & 1.30$\pm$0.30(-17) & 4.54(-18) & 14.30$\pm$2.00 & 10.53 & 101.77 \\
$\mathrm{OH}$ & 65.131 & 7.00$\pm$2.00(-17) & 4.02(-17) &  & 9.41 & 94.65 \\
$\mathrm{OH}$ & 65.278 & 1.25$\pm$0.20(-16) & 5.97(-17) &  & 7.21 & 96.21 \\
$\mathrm{OH}$ & 71.170 & 4.50$\pm$0.60(-17) & 2.18(-17) &  & 12.07 & 93.71 \\
$\mathrm{OH}$ & 71.215 & 4.50$\pm$0.60(-17) & 2.60(-17) &  & 10.28 & 95.25 \\
$\mathrm{OH}$ & 79.115 & 2.46$\pm$0.79(-17) & 2.36(-17) &  & 5.93 & 101.06 \\
$\mathrm{OH}$ & 79.179 & $<$2.40(-17) & 2.42(-17) &  & 5.97 & 101.16 \\
$\mathrm{OH}$ & 84.420 & 1.01$\pm$0.15(-16) & 5.42(-17) &  & 7.67 & 96.20 \\
$\mathrm{OH}$ & 84.596 & 1.01$\pm$0.15(-16) & 7.19(-17) &  & 7.23 & 97.72 \\
$\mathrm{OH}$ & 119.234 & 2.80$\pm$1.40(-17) & 3.73(-17) &  & 7.23 & 100.49 \\
$\mathrm{OH}$ & 119.441 & 3.10$\pm$1.40(-17) & 4.50(-17) &  & 7.01 & 103.81 \\
$\mathrm{o\!-\!H_2}$ & 17.033 & 6.90$\pm$2.60(-18) & 1.45(-16) & 7.75$\pm$1.25 & 8.54 & 139.60 \\
$\mathrm{p\!-\!H_2}$ & 12.277 & 5.60$\pm$2.00(-18) & 3.65(-17) & 8.30$\pm$1.20 & 7.84 & 113.47 \\
$\mathrm{p\!-\!H_2}$ & 8.025 & 1.47$\pm$0.34(-17) & 4.22(-18) & 10.40$\pm$2.00 & 5.97 & 111.03 \\
$\mathrm{o\!-\!H_2}$ & 4.694 & 9.00$\pm$2.00(-18) & 4.07(-19) & 15.90$\pm$2.00 & 11.14 & 102.35 \\
\hline
\end{tabular}


==> DIANAmodels/BPTau.tex <==
\centering\begin{tabular}{rr}
\hline
DIANA standard fit model properties &  \\
\hline
minimum dust temperature [K] & 4.09 \\
maximum dust temperature [K] & 1722.55 \\
mass-mean dust temperature [K] & 15.16 \\
minimum  gas temperature [K] & 4.18 \\
maximum  gas temperature [K] & 40000.00 \\
mass-mean  gas temperature [K] & 18.41 \\
mm-opacity-slope (0.85-1.3)mm & 1.37 \\
cm-opacity-slope (5-10)mm & 1.64 \\
mm-SED-slope (0.85-1.3)mm & 1.94 \\
cm-SED-slope (5-10)mm & 3.33 \\
10$\mathrm{\mu m}$ silicate emission amplitude & 1.71 \\
naked star luminosity [$L_\odot$] & 1.00 \\
bolometric luminosity [$L_\odot$] & 1.34 \\
near IR excess ($\lambda=$2.05-6.90$\mathrm{\mu m}$)
 [$L_\odot$] & 0.13 \\
mid IR excess ($\lambda=$6.90-29.3$\mathrm{\mu m}$)
 [$L_\odot$] & 0.10 \\
far IR excess ($\lambda=$29.3-970.$\mathrm{\mu m}$)
 [$L_\odot$] & 0.03 \\
\hline
\end{tabular}


\vspace{0.5cm}\centering\begin{tabular}{lrccccr}
\hline & & \multicolumn{2}{c}{line flux $[\mathrm{W\,m^{-2}}$]} & \multicolumn{2}{c}{FWHM[$\mathrm{km\,s^{-1}}$]} &  \\
species & $\lambda\,$[$\mathrm{\mu m}]$ & observed & model & observed & model & size[AU] \\
\hline
$\mathrm{CO}$ & 1300.403 & 8.70$\pm$2.00(-21) & 1.06(-20) & 4.20$\pm$0.42 & 2.85 & 125.01 \\
$\mathrm{^{13}CO}$ & 1360.227 & 1.10$\pm$0.50(-21) & 1.53(-21) &  & 3.81 & 76.18 \\
$\mathrm{CN}$ & 1321.390 & 2.40$\pm$0.50(-21) & 2.84(-22) &  & 2.59 & 143.38 \\
$\mathrm{CO}$ & 4.633 & 1.70$\pm$0.30(-17) & 1.18(-17) & 65.00$\pm$4.00 & 87.01 & 0.65 \\
$\mathrm{CO}$ & 4.477 & 1.90$\pm$0.20(-17) & 1.33(-17) & 70.00$\pm$3.00 & 88.36 & 0.35 \\
$\mathrm{OI}$ & 63.183 & 9.53$\pm$2.70(-18) & 2.69(-17) &  & 2.66 & 140.18 \\
$\mathrm{o\!-\!H_2O}$ & 63.323 & $<$9.30(-18) & 5.88(-19) &  & 27.40 & 1.22 \\
\hline
\end{tabular}


==> DIANAmodels/CYTau.tex <==
\centering\begin{tabular}{rr}
\hline
DIANA standard fit model properties &  \\
\hline
minimum dust temperature [K] & 4.79 \\
maximum dust temperature [K] & 1682.75 \\
mass-mean dust temperature [K] & 9.45 \\
minimum  gas temperature [K] & 4.79 \\
maximum  gas temperature [K] & 40000.00 \\
mass-mean  gas temperature [K] & 12.04 \\
mm-opacity-slope (0.85-1.3)mm & 1.26 \\
cm-opacity-slope (5-10)mm & 1.75 \\
mm-SED-slope (0.85-1.3)mm & 1.60 \\
cm-SED-slope (5-10)mm & 2.95 \\
10$\mathrm{\mu m}$ silicate emission amplitude & 1.61 \\
naked star luminosity [$L_\odot$] & 0.37 \\
bolometric luminosity [$L_\odot$] & 0.52 \\
near IR excess ($\lambda=$2.07-6.96$\mathrm{\mu m}$)
 [$L_\odot$] & 0.06 \\
mid IR excess ($\lambda=$6.96-29.5$\mathrm{\mu m}$)
 [$L_\odot$] & 0.03 \\
far IR excess ($\lambda=$29.5-973.$\mathrm{\mu m}$)
 [$L_\odot$] & 0.01 \\
\hline
\end{tabular}


\vspace{0.5cm}\centering\begin{tabular}{lrccccr}
\hline & & \multicolumn{2}{c}{line flux $[\mathrm{W\,m^{-2}}$]} & \multicolumn{2}{c}{FWHM[$\mathrm{km\,s^{-1}}$]} &  \\
species & $\lambda\,$[$\mathrm{\mu m}]$ & observed & model & observed & model & size[AU] \\
\hline
$\mathrm{CO}$ & 1300.403 & 1.63$\pm$0.30(-20) & 2.02(-20) & 2.35$\pm$0.20 & 2.27 & 199.68 \\
$\mathrm{^{13}CO}$ & 1360.227 & 7.81$\pm$0.90(-21) & 5.96(-21) & 2.55$\pm$0.22 & 2.57 & 199.35 \\
$\mathrm{OI}$ & 63.183 & 1.20$\pm$0.15(-17) & 5.60(-18) &  & 3.19 & 143.19 \\
$\mathrm{OI}$ & 0.630 & 7.80$\pm$0.50(-18) & 9.38(-18) & 42.00$\pm$3.00 & 58.98 & 0.45 \\
$\mathrm{o\!-\!H_2O}$ & 63.323 & $<$1.20(-17) & 1.44(-19) &  & 29.78 & 0.67 \\
$\mathrm{CO}$ & 4.633 & 6.00$\pm$2.00(-18) & 6.60(-18) & 75.00$\pm$11.00 & 13.96 & 4.08 \\
$\mathrm{CO}$ & 4.920 & 5.00$\pm$1.00(-18) & 4.20(-18) & 86.00$\pm$9.00 & 92.12 & 0.15 \\
\hline
\end{tabular}


==> DIANAmodels/DMTau.tex <==
\centering\begin{tabular}{rr}
\hline
DIANA standard fit model properties &  \\
\hline
minimum dust temperature [K] & 4.59 \\
maximum dust temperature [K] & 241.78 \\
mass-mean dust temperature [K] & 9.17 \\
minimum  gas temperature [K] & 4.78 \\
maximum  gas temperature [K] & 15977.99 \\
mass-mean  gas temperature [K] & 13.28 \\
mm-opacity-slope (0.85-1.3)mm & 0.98 \\
cm-opacity-slope (5-10)mm & 1.29 \\
mm-SED-slope (0.85-1.3)mm & 2.13 \\
cm-SED-slope (5-10)mm & 3.07 \\
10$\mathrm{\mu m}$ silicate emission amplitude & 2.03 \\
naked star luminosity [$L_\odot$] & 0.28 \\
bolometric luminosity [$L_\odot$] & 0.36 \\
near IR excess ($\lambda=$2.02-6.72$\mathrm{\mu m}$)
 [$L_\odot$] & 0.00 \\
mid IR excess ($\lambda=$6.72-29.5$\mathrm{\mu m}$)
 [$L_\odot$] & 0.02 \\
far IR excess ($\lambda=$29.5-991.$\mathrm{\mu m}$)
 [$L_\odot$] & 0.04 \\
\hline
\end{tabular}


\vspace{0.5cm}\centering\begin{tabular}{lrccccr}
\hline & & \multicolumn{2}{c}{line flux $[\mathrm{W\,m^{-2}}$]} & \multicolumn{2}{c}{FWHM[$\mathrm{km\,s^{-1}}$]} &  \\
species & $\lambda\,$[$\mathrm{\mu m}]$ & observed & model & observed & model & size[AU] \\
\hline
$\mathrm{Ne^+}$ & 12.814 & 5.50$\pm$1.10(-18) & 3.32(-17) &  & 15.31 & 7.43 \\
$\mathrm{OI}$ & 63.183 & 7.00$\pm$2.00(-18) & 4.61(-17) &  & 2.97 & 331.60 \\
$\mathrm{OI}$ & 145.525 & $<$3.60(-18) & 1.23(-18) &  & 8.53 & 164.31 \\
$\mathrm{CII}$ & 157.740 & $<$3.60(-18) & 4.54(-18) &  & 1.52 & 565.04 \\
$\mathrm{o\!-\!H_2O}$ & 63.323 & $<$5.40(-18) & 8.76(-19) &  & 9.25 & 11.89 \\
$\mathrm{CO}$ & 866.963 & 1.93$\pm$0.11(-19) & 3.74(-19) &  & 1.80 & 448.90 \\
$\mathrm{CO}$ & 1300.404 & 1.14$\pm$0.31(-19) & 1.16(-19) &  & 1.79 & 443.90 \\
$\mathrm{^{13}CO}$ & 1360.227 & 3.97$\pm$0.48(-20) & 1.77(-20) &  & 2.19 & 324.32 \\
$\mathrm{C^{18}O}$ & 1365.421 & 4.98$\pm$0.51(-21) & 3.78(-21) &  & 2.37 & 289.54 \\
$\mathrm{CN}$ & 881.097 & 6.74$\pm$0.67(-20) & 1.57(-19) &  & 1.70 & 470.52 \\
$\mathrm{CN}$ & 1321.390 & 3.59$\pm$0.30(-20) & 6.49(-20) &  & 1.63 & 482.01 \\
$\mathrm{HCN}$ & 845.663 & 1.92$\pm$0.19(-20) & 1.16(-19) &  & 1.82 & 415.29 \\
$\mathrm{HCN}$ & 1127.520 & 2.58$\pm$0.49(-20) & 7.55(-20) &  & 1.73 & 440.48 \\
$\mathrm{HCO^+}$ & 840.380 & 7.55$\pm$0.43(-20) & 7.21(-20) &  & 1.85 & 439.81 \\
$\mathrm{HCO^+}$ & 1120.478 & 4.77$\pm$0.11(-20) & 4.43(-20) &  & 1.72 & 461.83 \\
$\mathrm{N_2H^+}$ & 804.439 & $<$6.72(-21) & 1.15(-20) &  & 2.05 & 273.25 \\
$\mathrm{N_2H^+}$ & 1072.557 & 9.32$\pm$0.93(-21) & 7.13(-21) &  & 2.02 & 289.61 \\
\hline
\end{tabular}


==> DIANAmodels/GMAur.tex <==
\centering\begin{tabular}{rr}
\hline
DIANA standard fit model properties &  \\
\hline
minimum dust temperature [K] & 5.79 \\
maximum dust temperature [K] & 885.86 \\
mass-mean dust temperature [K] & 17.86 \\
minimum  gas temperature [K] & 7.42 \\
maximum  gas temperature [K] & 26157.07 \\
mass-mean  gas temperature [K] & 18.58 \\
mm-opacity-slope (0.85-1.3)mm & 1.30 \\
cm-opacity-slope (5-10)mm & 1.67 \\
mm-SED-slope (0.85-1.3)mm & 2.35 \\
cm-SED-slope (5-10)mm & 3.52 \\
10$\mathrm{\mu m}$ silicate emission amplitude & 1.84 \\
naked star luminosity [$L_\odot$] & 0.68 \\
bolometric luminosity [$L_\odot$] & 0.94 \\
near IR excess ($\lambda=$2.07-6.84$\mathrm{\mu m}$)
 [$L_\odot$] & 0.03 \\
mid IR excess ($\lambda=$6.84-29.9$\mathrm{\mu m}$)
 [$L_\odot$] & 0.05 \\
far IR excess ($\lambda=$29.9-998.$\mathrm{\mu m}$)
 [$L_\odot$] & 0.14 \\
\hline
\end{tabular}


\vspace{0.5cm}\centering\begin{tabular}{lrccccr}
\hline & & \multicolumn{2}{c}{line flux $[\mathrm{W\,m^{-2}}$]} & \multicolumn{2}{c}{FWHM[$\mathrm{km\,s^{-1}}$]} &  \\
species & $\lambda\,$[$\mathrm{\mu m}]$ & observed & model & observed & model & size[AU] \\
\hline
$\mathrm{OI}$ & 0.630 & 3.90$\pm$1.00(-17) & 1.23(-17) & 42.00$\pm$0.00 & 10.41 & 27.48 \\
$\mathrm{CO}$ & 4.649 & 1.30$\pm$0.90(-18) & 1.25(-16) & 22.80$\pm$0.00 & 9.05 & 19.42 \\
$\mathrm{CO}$ & 4.657 & 9.00$\pm$8.00(-19) & 8.30(-17) & 15.60$\pm$0.00 & 9.08 & 19.44 \\
$\mathrm{CO}$ & 4.699 & 1.00$\pm$0.80(-18) & 1.98(-16) & 19.60$\pm$0.00 & 9.05 & 19.43 \\
$\mathrm{CO}$ & 4.708 & 1.10$\pm$0.80(-18) & 1.93(-16) & 18.00$\pm$0.00 & 9.08 & 19.43 \\
$\mathrm{CO}$ & 4.717 & 1.10$\pm$0.80(-18) & 1.68(-16) & 18.00$\pm$0.00 & 9.08 & 19.45 \\
$\mathrm{CO}$ & 4.726 & 1.50$\pm$0.90(-18) & 1.32(-16) & 26.90$\pm$0.00 & 9.08 & 19.45 \\
$\mathrm{CO}$ & 4.735 & 1.60$\pm$0.90(-18) & 9.69(-17) & 25.40$\pm$0.00 & 9.08 & 19.47 \\
$\mathrm{CO}$ & 4.745 & 2.20$\pm$1.10(-18) & 6.70(-17) & 37.20$\pm$0.00 & 9.08 & 19.48 \\
$\mathrm{CO}$ & 4.754 & 2.70$\pm$1.20(-18) & 4.48(-17) & 44.60$\pm$0.00 & 9.08 & 19.50 \\
$\mathrm{CO}$ & 4.763 & 2.30$\pm$1.10(-18) & 2.96(-17) & 35.60$\pm$0.00 & 9.08 & 19.53 \\
$\mathrm{CO}$ & 4.773 & 2.90$\pm$1.20(-18) & 1.96(-17) & 42.90$\pm$0.00 & 9.08 & 19.59 \\
$\mathrm{CO}$ & 4.793 & 2.80$\pm$1.20(-18) & 9.06(-18) & 46.30$\pm$0.00 & 9.11 & 19.73 \\
$\mathrm{Ne^+}$ & 12.814 & 1.20$\pm$0.30(-17) & 6.78(-18) &  & 9.52 & 53.27 \\
$\mathrm{OI}$ & 63.183 & 3.79$\pm$0.51(-17) & 7.25(-17) &  & 5.44 & 230.21 \\
$\mathrm{o\!-\!H_2O}$ & 63.323 & $<$7.27(-18) & 4.34(-18) &  & 9.13 & 20.18 \\
$\mathrm{CO}$ & 1300.404 & 1.49$\pm$0.28(-19) & 1.00(-19) &  & 2.74 & 402.84 \\
$\mathrm{HCO^+}$ & 1120.478 & 3.85$\pm$0.13(-20) & 1.20(-20) &  & 3.49 & 346.65 \\
\hline
\end{tabular}


==> DIANAmodels/HD142666.tex <==
\centering\begin{tabular}{rr}
\hline
DIANA standard fit model properties &  \\
\hline
minimum dust temperature [K] & 7.19 \\
maximum dust temperature [K] & 1890.40 \\
mass-mean dust temperature [K] & 24.79 \\
minimum  gas temperature [K] & 10.17 \\
maximum  gas temperature [K] & 24910.24 \\
mass-mean  gas temperature [K] & 34.25 \\
mm-opacity-slope (0.85-1.3)mm & 0.60 \\
cm-opacity-slope (5-10)mm & 0.93 \\
mm-SED-slope (0.85-1.3)mm & 2.22 \\
cm-SED-slope (5-10)mm & 2.80 \\
10$\mathrm{\mu m}$ silicate emission amplitude & 1.77 \\
naked star luminosity [$L_\odot$] & 6.33 \\
bolometric luminosity [$L_\odot$] & 9.05 \\
near IR excess ($\lambda=$2.02-6.72$\mathrm{\mu m}$)
 [$L_\odot$] & 0.81 \\
mid IR excess ($\lambda=$6.72-29.5$\mathrm{\mu m}$)
 [$L_\odot$] & 0.60 \\
far IR excess ($\lambda=$29.5-991.$\mathrm{\mu m}$)
 [$L_\odot$] & 0.22 \\
\hline
\end{tabular}


\vspace{0.5cm}\centering\begin{tabular}{lrccccr}
\hline & & \multicolumn{2}{c}{line flux $[\mathrm{W\,m^{-2}}$]} & \multicolumn{2}{c}{FWHM[$\mathrm{km\,s^{-1}}$]} &  \\
species & $\lambda\,$[$\mathrm{\mu m}]$ & observed & model & observed & model & size[AU] \\
\hline
$\mathrm{CO}$ & 1300.404 & 1.05$\pm$0.11(-19) & 7.63(-20) & 6.37$\pm$1.32 & 4.25 & 245.19 \\
$\mathrm{CO}$ & 2600.758 & 4.41$\pm$0.36(-20) & 8.87(-21) & 10.63$\pm$1.32 & 4.42 & 231.57 \\
$\mathrm{CO}$ & 72.842 & $<$3.00(-17) & 4.97(-20) &  & 122.42 & 0.59 \\
$\mathrm{CO}$ & 130.368 & $<$1.19(-17) & 1.01(-18) &  & 27.73 & 9.28 \\
$\mathrm{OI}$ & 63.183 & 1.89$\pm$0.31(-17) & 1.67(-17) &  & 21.19 & 46.75 \\
$\mathrm{OI}$ & 145.525 & $<$4.70(-18) & 1.93(-18) &  & 15.36 & 39.93 \\
$\mathrm{CII}$ & 157.740 & $<$9.00(-18) & 1.22(-18) &  & 3.60 & 304.80 \\
$\mathrm{CO}$ & 72.842 & $<$1.63(-17) & 4.97(-20) &  & 122.42 & 0.59 \\
$\mathrm{CO}$ & 79.359 & $<$1.88(-17) & 8.55(-20) &  & 104.12 & 0.85 \\
$\mathrm{CO}$ & 90.162 & $<$1.26(-17) & 1.75(-19) &  & 79.53 & 1.79 \\
$\mathrm{CO}$ & 144.784 & $<$6.18(-18) & 1.19(-18) &  & 22.96 & 11.46 \\
$\mathrm{CO}$ & 4.652 & $<$5.60(-18) & 9.32(-18) &  & 146.10 & 1.84 \\
$\mathrm{CO}$ & 4.990 & $<$3.09(-18) & 4.38(-18) &  & 146.24 & 0.16 \\
\hline
\end{tabular}


==> DIANAmodels/HD163296.tex <==
\centering\begin{tabular}{rr}
\hline
DIANA standard fit model properties &  \\
\hline
minimum dust temperature [K] & 9.72 \\
maximum dust temperature [K] & 1945.93 \\
mass-mean dust temperature [K] & 27.29 \\
minimum  gas temperature [K] & 12.34 \\
maximum  gas temperature [K] & 15202.64 \\
mass-mean  gas temperature [K] & 28.75 \\
mm-opacity-slope (0.85-1.3)mm & 1.39 \\
cm-opacity-slope (5-10)mm & 1.65 \\
mm-SED-slope (0.85-1.3)mm & 2.47 \\
cm-SED-slope (5-10)mm & 3.09 \\
10$\mathrm{\mu m}$ silicate emission amplitude & 2.04 \\
naked star luminosity [$L_\odot$] & 34.42 \\
bolometric luminosity [$L_\odot$] & 48.72 \\
near IR excess ($\lambda=$2.05-6.90$\mathrm{\mu m}$)
 [$L_\odot$] & 4.10 \\
mid IR excess ($\lambda=$6.90-29.3$\mathrm{\mu m}$)
 [$L_\odot$] & 2.18 \\
far IR excess ($\lambda=$29.3-970.$\mathrm{\mu m}$)
 [$L_\odot$] & 0.70 \\
\hline
\end{tabular}


\vspace{0.5cm}\centering\begin{tabular}{lrccccr}
\hline & & \multicolumn{2}{c}{line flux $[\mathrm{W\,m^{-2}}$]} & \multicolumn{2}{c}{FWHM[$\mathrm{km\,s^{-1}}$]} &  \\
species & $\lambda\,$[$\mathrm{\mu m}]$ & observed & model & observed & model & size[AU] \\
\hline
$\mathrm{CO}$ & 72.842 & $<$1.07(-17) & 3.23(-18) &  & 51.92 & 2.89 \\
$\mathrm{CO}$ & 79.359 & $<$1.55(-17) & 3.61(-18) &  & 49.23 & 2.99 \\
$\mathrm{CO}$ & 90.162 & $<$7.38(-18) & 3.37(-18) &  & 48.13 & 3.06 \\
$\mathrm{CO}$ & 144.784 & 6.70$\pm$1.50(-18) & 2.84(-18) &  & 20.14 & 55.20 \\
$\mathrm{CO}$ & 866.963 & 1.11$\pm$0.04(-18) & 1.27(-18) & 4.48$\pm$0.10 & 4.45 & 388.79 \\
$\mathrm{CO}$ & 1300.404 & 4.04$\pm$0.08(-19) & 3.66(-19) & 4.46$\pm$0.22 & 4.50 & 380.88 \\
$\mathrm{^{13}CO}$ & 1360.227 & 1.38$\pm$0.22(-19) & 1.23(-19) & 4.90$\pm$0.32 & 4.89 & 313.24 \\
$\mathrm{C^{18}O}$ & 1365.421 & 4.52$\pm$0.18(-20) & 5.42(-20) & 5.48$\pm$0.32 & 5.31 & 284.18 \\
$\mathrm{^{13}CO}$ & 2720.406 & 1.24$\pm$0.70(-20) & 1.08(-20) & 4.50$\pm$0.50 & 5.16 & 279.95 \\
$\mathrm{OI}$ & 63.183 & 1.71$\pm$0.15(-16) & 5.30(-16) &  & 4.17 & 447.07 \\
$\mathrm{OI}$ & 145.525 & $<$6.00(-18) & 4.68(-17) &  & 4.11 & 407.01 \\
$\mathrm{o\!-\!H_2O}$ & 29.836 & 4.34$\pm$0.39(-17) & 4.81(-17) &  & 49.48 & 3.13 \\
$\mathrm{o\!-\!H_2O}$ & 63.323 & 1.57$\pm$0.36(-17) & 1.09(-17) &  & 50.27 & 3.18 \\
$\mathrm{p\!-\!H_2O}$ & 63.458 & 1.11$\pm$0.32(-17) & 1.03(-17) &  & 50.27 & 3.13 \\
$\mathrm{o\!-\!H_2O}$ & 71.946 & 1.38$\pm$0.54(-17) & 8.05(-18) &  & 50.15 & 3.27 \\
$\mathrm{o\!-\!H_2O}$ & 78.742 & 1.07$\pm$0.35(-17) & 6.65(-18) &  & 50.09 & 6.91 \\
$\mathrm{p\!-\!H_2O}$ & 78.928 & $<$1.41(-17) & 5.78(-18) &  & 50.21 & 3.16 \\
$\mathrm{p\!-\!H_2O}$ & 89.988 & $<$5.10(-18) & 5.32(-18) &  & 4.43 & 264.90 \\
$\mathrm{p\!-\!H_2O}$ & 144.517 & $<$1.22(-17) & 1.10(-18) &  & 49.91 & 3.42 \\
$\mathrm{p\!-\!H_2O}$ & 158.311 & $<$1.37(-17) & 6.75(-19) &  & 49.60 & 3.08 \\
$\mathrm{o\!-\!H_2O}$ & 179.526 & $<$1.67(-17) & 1.09(-17) &  & 4.86 & 336.59 \\
$\mathrm{o\!-\!H_2O}$ & 180.488 & $<$1.67(-17) & 2.47(-18) &  & 4.61 & 318.79 \\
$\mathrm{OH}$ & 79.115 & 1.17$\pm$0.30(-17) & 2.76(-18) &  & 47.28 & 93.62 \\
$\mathrm{OH}$ & 79.179 & $<$9.00(-18) & 2.78(-18) &  & 46.30 & 119.99 \\
$\mathrm{CO}$ & 650.251 & $<$2.07(-17) & 2.95(-18) &  & 4.42 & 386.25 \\
$\mathrm{CO}$ & 520.231 & 1.04$\pm$0.40(-17) & 5.46(-18) &  & 4.41 & 388.61 \\
$\mathrm{CO}$ & 433.556 & 7.40$\pm$2.90(-18) & 8.74(-18) &  & 4.38 & 389.13 \\
$\mathrm{CO}$ & 371.650 & 9.00$\pm$3.00(-18) & 1.26(-17) &  & 4.36 & 387.93 \\
$\mathrm{CO}$ & 325.225 & 1.24$\pm$0.56(-17) & 1.66(-17) &  & 4.34 & 385.30 \\
$\mathrm{CO}$ & 289.120 & 9.10$\pm$3.80(-18) & 2.02(-17) &  & 4.34 & 381.19 \\
$\mathrm{CO}$ & 260.239 & 1.17$\pm$0.34(-17) & 2.24(-17) &  & 4.36 & 375.02 \\
$\mathrm{CO}$ & 236.613 & 1.13$\pm$0.29(-17) & 2.15(-17) &  & 4.42 & 367.78 \\
$\mathrm{CO}$ & 216.927 & 1.17$\pm$0.34(-17) & 1.70(-17) &  & 4.51 & 361.75 \\
$\mathrm{CO}$ & 200.272 & 1.52$\pm$0.37(-17) & 1.20(-17) &  & 5.98 & 352.74 \\
$\mathrm{C}$ & 370.415 & 5.00$\pm$2.00(-18) & 4.88(-18) &  & 4.15 & 418.41 \\
$\mathrm{N^+}$ & 205.240 & 1.70$\pm$0.20(-17) & 4.53(-22) &  & 5.82 & 478.39 \\
\hline
\end{tabular}

==> DIANAmodels/HD169142-2.tex <==
\centering\begin{tabular}{rr}
\hline
DIANA standard fit model properties &  \\
\hline
minimum dust temperature [K] & 12 \\
maximum dust temperature [K] & 2325 \\
mass-mean dust temperature [K] & 28 \\
minimum  gas temperature [K] & 14 \\
maximum  gas temperature [K] & 40000 \\
mass-mean  gas temperature [K] & 36 \\
mm-opacity-slope (0.85-1.3)mm & 1.0 \\
cm-opacity-slope (5-10)mm & 1.2 \\
mm-SED-slope (0.85-1.3)mm & 2.8 \\
cm-SED-slope (5-10)mm & 3.2 \\
10$\mathrm{\mu m}$ silicate emission amplitude & 1.6 \\
naked star luminosity [$L_\odot$] & 10.0 \\
bolometric luminosity [$L_\odot$] & 13.7 \\
near IR excess ($\lambda=$2.02-6.72$\mathrm{\mu m}$)
 [$L_\odot$] & 0.88 \\
mid IR excess ($\lambda=$6.72-29.5$\mathrm{\mu m}$)
 [$L_\odot$] & 0.81 \\
far IR excess ($\lambda=$29.5-991.$\mathrm{\mu m}$)
 [$L_\odot$] & 0.99 \\
\hline
\end{tabular}


\vspace{0.5cm}\centering\begin{tabular}{lrccccr}
\hline & & \multicolumn{2}{c}{line flux $[\mathrm{W\,m^{-2}}$]} & \multicolumn{2}{c}{FWHM $[\mathrm{km\,s^{-1}}]$} &  \\
species & $\lambda\,$[$\mathrm{\mu m}]$ & observed & model & observed & model & size[AU] \\
\hline
$\mathrm{OI}$ & 63.183 & 7.2$\pm$0.4(-17) & 4.5(-17) &  & 3.2 & 121.8 \\
$\mathrm{OI}$ & 145.525 & $<$1.1(-17) & 1.6(-18) &  & 3.7 & 72.8 \\
$\mathrm{CII}$ & 157.740 & $<$6.6(-18) & 2.8(-18) &  & 1.2 & 436.4 \\
$\mathrm{CO}$ & 1300.404 & 9.3$\pm$0.4(-20) & 1.7(-19) & 2.1$\pm$0.1 & 1.4 & 415.8 \\
$\mathrm{^{13}CO}$ & 1360.227 & 4.8$\pm$0.4(-20) & 4.2(-20) & 2.1$\pm$0.1 & 1.6 & 323.6 \\
$\mathrm{C^{18}O}$ & 1365.421 & 2.0$\pm$0.4(-20) & 1.0(-20) &  & 1.7 & 299.1 \\
$\mathrm{o\!-\!H_2O}$ & 179.526 & $<$8.7(-18) & 1.5(-17) &  & 2.3 & 338.7 \\
$\mathrm{o\!-\!H_2O}$ & 78.742 & $<$1.1(-17) & 1.9(-17) &  & 3.2 & 125.1 \\
$\mathrm{CO}$ & 72.842 & $<$1.6(-17) & 2.6(-20) &  & 4.1 & 23.6 \\
$\mathrm{CO}$ & 90.162 & $<$1.1(-17) & 5.4(-19) &  & 4.1 & 24.0 \\
$\mathrm{CO}$ & 4.754 & 2.5$\pm$0.1(-18) & 2.0(-17) & 7.1$\pm$0.4 & 3.8 & 22.1 \\
$\mathrm{CO}$ & 4.773 & 2.2$\pm$0.1(-18) & 1.4(-17) & 6.5$\pm$0.4 & 3.8 & 22.1 \\
\hline
\end{tabular}

==> DIANAmodels/HD169142.tex <==
\centering\begin{tabular}{rr}
\hline
DIANA standard fit model properties &  \\
\hline
minimum dust temperature [K] & 11.58 \\
maximum dust temperature [K] & 2325.49 \\
mass-mean dust temperature [K] & 28.03 \\
minimum  gas temperature [K] & 13.79 \\
maximum  gas temperature [K] & 40000.00 \\
mass-mean  gas temperature [K] & 36.28 \\
mm-opacity-slope (0.85-1.3)mm & 1.02 \\
cm-opacity-slope (5-10)mm & 1.23 \\
mm-SED-slope (0.85-1.3)mm & 2.76 \\
cm-SED-slope (5-10)mm & 3.19 \\
10$\mathrm{\mu m}$ silicate emission amplitude & 1.61 \\
naked star luminosity [$L_\odot$] & 9.95 \\
bolometric luminosity [$L_\odot$] & 13.75 \\
near IR excess ($\lambda=$2.02-6.72$\mathrm{\mu m}$)
 [$L_\odot$] & 0.88 \\
mid IR excess ($\lambda=$6.72-29.5$\mathrm{\mu m}$)
 [$L_\odot$] & 0.81 \\
far IR excess ($\lambda=$29.5-991.$\mathrm{\mu m}$)
 [$L_\odot$] & 0.99 \\
\hline
\end{tabular}


\vspace{0.5cm}\centering\begin{tabular}{lrccccr}
\hline & & \multicolumn{2}{c}{line flux $[\mathrm{W\,m^{-2}}$]} & \multicolumn{2}{c}{FWHM[$\mathrm{km\,s^{-1}}$]} &  \\
species & $\lambda\,$[$\mathrm{\mu m}]$ & observed & model & observed & model & size[AU] \\
\hline
$\mathrm{OI}$ & 63.183 & 7.17$\pm$0.38(-17) & 4.47(-17) &  & 3.17 & 121.75 \\
$\mathrm{OI}$ & 145.525 & $<$1.05(-17) & 1.56(-18) &  & 3.67 & 72.76 \\
$\mathrm{CII}$ & 157.740 & $<$6.60(-18) & 2.84(-18) &  & 1.21 & 436.37 \\
$\mathrm{CO}$ & 1300.404 & 9.30$\pm$0.40(-20) & 1.67(-19) & 2.10$\pm$0.10 & 1.42 & 415.78 \\
$\mathrm{^{13}CO}$ & 1360.227 & 4.80$\pm$0.40(-20) & 4.21(-20) & 2.10$\pm$0.10 & 1.59 & 323.61 \\
$\mathrm{C^{18}O}$ & 1365.421 & 2.00$\pm$0.40(-20) & 1.02(-20) &  & 1.68 & 299.14 \\
$\mathrm{o\!-\!H_2O}$ & 179.526 & $<$8.70(-18) & 1.47(-17) &  & 2.31 & 338.69 \\
$\mathrm{o\!-\!H_2O}$ & 78.742 & $<$1.05(-17) & 1.93(-17) &  & 3.24 & 125.07 \\
$\mathrm{CO}$ & 72.842 & $<$1.56(-17) & 2.58(-20) &  & 4.06 & 23.58 \\
$\mathrm{CO}$ & 90.162 & $<$1.05(-17) & 5.36(-19) &  & 4.06 & 24.02 \\
$\mathrm{CO}$ & 4.754 & 2.50$\pm$0.10(-18) & 1.97(-17) & 7.10$\pm$0.40 & 3.84 & 22.09 \\
$\mathrm{CO}$ & 4.773 & 2.20$\pm$0.10(-18) & 1.38(-17) & 6.50$\pm$0.40 & 3.84 & 22.10 \\
\hline
\end{tabular}


==> DIANAmodels/LkCa15-2.tex <==
\begin{table}\centering\begin{tabular}{rr}
\hline
DIANA standard fit model properties &  \\
\hline
minimum dust temperature [K] & 6 \\
maximum dust temperature [K] & 1538 \\
mass-mean dust temperature [K] & 12 \\
minimum  gas temperature [K] & 6 \\
maximum  gas temperature [K] & 27008 \\
mass-mean  gas temperature [K] & 18 \\
mm-opacity-slope (0.85-1.3)mm & 1.2 \\
cm-opacity-slope (5-10)mm & 1.8 \\
mm-SED-slope (0.85-1.3)mm & 2.4 \\
cm-SED-slope (5-10)mm & 3.5 \\
10$\mathrm{\mu m}$ silicate emission amplitude & 2.2 \\
naked star luminosity [$L_\odot$] & 1.4 \\
bolometric luminosity [$L_\odot$] & 1.6 \\
near IR excess ($\lambda=$2.02-6.72$\mathrm{\mu m}$)
 [$L_\odot$] & 0.06 \\
mid IR excess ($\lambda=$6.72-29.5$\mathrm{\mu m}$)
 [$L_\odot$] & 0.05 \\
far IR excess ($\lambda=$29.5-991.$\mathrm{\mu m}$)
 [$L_\odot$] & 0.07 \\
\hline
\end{tabular}


\vspace{0.5cm}\centering\begin{tabular}{lrccccr}
\hline & & \multicolumn{2}{c}{line flux $[\mathrm{W\,m^{-2}}$]} & \multicolumn{2}{c}{FWHM $[\mathrm{km\,s^{-1}}]$} &  \\
species & $\lambda\,$[$\mathrm{\mu m}]$ & observed & model & observed & model & size[AU] \\
\hline
$\mathrm{OI}$ & 63.183 & 1.0$\pm$0.2(-17) & 8.4(-17) &  & 6.7 & 161.2 \\
$\mathrm{OI}$ & 145.525 & $<$9.0(-18) & 2.6(-18) &  & 7.0 & 102.7 \\
$\mathrm{CII}$ & 157.740 & $<$1.1(-17) & 3.8(-18) &  & 3.5 & 312.5 \\
$\mathrm{CO}$ & 1300.404 & 8.7$\pm$0.2(-20) & 7.6(-20) & 2.8$\pm$0.1 & 3.6 & 269.5 \\
$\mathrm{^{13}CO}$ & 1360.227 & 3.2$\pm$0.2(-20) & 2.6(-20) & 2.9$\pm$0.3 & 3.9 & 220.2 \\
$\mathrm{C^{18}O}$ & 1365.421 & 5.3$\pm$0.4(-21) & 9.3(-21) &  & 4.3 & 201.2 \\
$\mathrm{HCO^+}$ & 1120.478 & 4.7$\pm$0.2(-20) & 2.9(-20) & 3.3$\pm$0.2 & 3.2 & 289.4 \\
$\mathrm{HCN}$ & 1127.520 & 5.1$\pm$0.3(-20) & 4.1(-20) & 4.0$\pm$0.3 & 3.2 & 300.4 \\
$\mathrm{CS}$ & 1223.964 & 1.2$\pm$0.2(-20) & 6.1(-21) & 3.4$\pm$0.6 & 3.2 & 265.6 \\
$\mathrm{o\!-\!H_2CO}$ & 1419.394 & 9.4$\pm$0.5(-21) & 1.2(-20) &  & 2.9 & 337.3 \\
$\mathrm{p\!-\!H_2CO}$ & 1373.794 & 5.4$\pm$0.5(-21) & 1.4(-20) &  & 2.9 & 339.0 \\
$\mathrm{o\!-\!H_2CO}$ & 1328.291 & 8.0$\pm$0.4(-21) & 1.4(-20) & 2.7$\pm$0.4 & 2.9 & 335.1 \\
$\mathrm{CO}$ & 433.556 & 6.2$\pm$0.3(-19) & 1.3(-18) & 5.4$\pm$0.5 & 3.8 & 243.2 \\
$\mathrm{HCO^+}$ & 840.380 & 1.4$\pm$0.1(-19) & 5.8(-20) & 3.4$\pm$0.2 & 3.3 & 273.9 \\
\hline
\end{tabular}
\end{table}

==> DIANAmodels/MWC480.tex <==
\centering\begin{tabular}{rr}
\hline
DIANA standard fit model properties &  \\
\hline
minimum dust temperature [K] & 10.84 \\
maximum dust temperature [K] & 1598.97 \\
mass-mean dust temperature [K] & 24.00 \\
minimum  gas temperature [K] & 10.88 \\
maximum  gas temperature [K] & 23864.65 \\
mass-mean  gas temperature [K] & 35.63 \\
mm-opacity-slope (0.85-1.3)mm & 1.04 \\
cm-opacity-slope (5-10)mm & 1.32 \\
mm-SED-slope (0.85-1.3)mm & 2.41 \\
cm-SED-slope (5-10)mm & n.a. \\
10$\mathrm{\mu m}$ silicate emission amplitude & 1.57 \\
naked star luminosity [$L_\odot$] & 13.34 \\
bolometric luminosity [$L_\odot$] & 20.33 \\
near IR excess ($\lambda=$2.05-6.82$\mathrm{\mu m}$)
 [$L_\odot$] & 2.88 \\
mid IR excess ($\lambda=$6.82-29.1$\mathrm{\mu m}$)
 [$L_\odot$] & 1.68 \\
far IR excess ($\lambda=$29.1-981.$\mathrm{\mu m}$)
 [$L_\odot$] & 0.58 \\
\hline
\end{tabular}


\vspace{0.5cm}\centering\begin{tabular}{lrccccr}
\hline & & \multicolumn{2}{c}{line flux $[\mathrm{W\,m^{-2}}$]} & \multicolumn{2}{c}{FWHM[$\mathrm{km\,s^{-1}}$]} &  \\
species & $\lambda\,$[$\mathrm{\mu m}]$ & observed & model & observed & model & size[AU] \\
\hline
$\mathrm{OI}$ & 63.183 & 9.49$\pm$0.35(-17) & 1.13(-16) &  & 8.27 & 151.56 \\
$\mathrm{OI}$ & 145.525 & $<$7.80(-18) & 7.91(-18) &  & 7.54 & 117.41 \\
$\mathrm{CII}$ & 157.740 & $<$9.60(-18) & 6.82(-18) &  & 3.17 & 410.35 \\
$\mathrm{CO}$ & 4.633 & 3.10$\pm$0.62(-17) & 3.97(-17) & 47.50$\pm$10.00 & 94.04 & 6.13 \\
$\mathrm{CO}$ & 4.641 & 3.20$\pm$0.64(-17) & 3.56(-17) & 53.70$\pm$10.00 & 93.75 & 8.24 \\
$\mathrm{CO}$ & 4.682 & 3.70$\pm$0.74(-17) & 2.90(-17) & 69.20$\pm$14.00 & 92.88 & 15.28 \\
$\mathrm{CO}$ & 4.726 & 3.60$\pm$0.72(-17) & 4.68(-17) & 48.10$\pm$10.00 & 93.17 & 7.82 \\
$\mathrm{CO}$ & 4.735 & 3.60$\pm$0.72(-17) & 4.80(-17) & 47.60$\pm$10.00 & 93.46 & 6.21 \\
$\mathrm{CO}$ & 4.920 & 3.40$\pm$0.68(-17) & 4.32(-17) & 69.90$\pm$13.40 & 95.49 & 0.28 \\
$\mathrm{CO}$ & 4.966 & 2.70$\pm$0.54(-17) & 4.09(-17) & 71.00$\pm$14.20 & 95.49 & 0.28 \\
$\mathrm{CO}$ & 4.990 & 3.20$\pm$0.64(-17) & 3.97(-17) & 80.00$\pm$16.00 & 95.49 & 0.28 \\
$\mathrm{CO}$ & 72.842 & $<$9.60(-18) & 2.65(-20) &  & 37.40 & 7.55 \\
$\mathrm{CO}$ & 79.359 & $<$1.62(-17) & 4.37(-20) &  & 33.92 & 8.99 \\
$\mathrm{CO}$ & 90.162 & $<$9.60(-18) & 1.37(-19) &  & 26.80 & 12.13 \\
$\mathrm{CO}$ & 144.784 & 6.90$\pm$3.20(-18) & 3.23(-18) &  & 10.82 & 50.26 \\
$\mathrm{CO}$ & 866.963 & 6.11$\pm$0.14(-19) & 5.65(-19) &  & 3.60 & 350.63 \\
$\mathrm{^{13}CO}$ & 906.846 & 1.14$\pm$0.23(-19) & 2.47(-19) &  & 4.12 & 275.89 \\
$\mathrm{CO}$ & 1300.404 & 1.69$\pm$0.05(-19) & 1.73(-19) &  & 3.65 & 346.49 \\
$\mathrm{o\!-\!H_2O}$ & 63.323 & $<$6.60(-18) & 9.13(-19) &  & 34.10 & 7.14 \\
$\mathrm{o\!-\!H_2O}$ & 71.946 & $<$1.23(-18) & 9.11(-19) &  & 30.36 & 9.31 \\
$\mathrm{o\!-\!H_2O}$ & 78.742 & $<$1.77(-17) & 1.66(-18) &  & 16.98 & 35.55 \\
$\mathrm{OH}$ & 79.115 & $<$9.90(-18) & 2.05(-18) &  & 8.47 & 106.56 \\
$\mathrm{OH}$ & 79.179 & $<$1.02(-17) & 2.13(-18) &  & 8.33 & 110.16 \\
$\mathrm{CN}$ & 881.097 & 6.74$\pm$0.67(-20) & 1.64(-20) &  & 3.13 & 394.95 \\
$\mathrm{CN}$ & 1321.390 & 2.49$\pm$0.11(-20) & 7.39(-21) &  & 3.00 & 388.94 \\
$\mathrm{HCN}$ & 845.663 & 3.57$\pm$0.36(-20) & 9.10(-20) &  & 4.02 & 294.78 \\
$\mathrm{HCN}$ & 1127.520 & 2.08$\pm$0.17(-20) & 4.52(-20) &  & 3.83 & 325.37 \\
$\mathrm{HCO^+}$ & 840.380 & 7.55$\pm$1.51(-20) & 1.02(-19) &  & 4.32 & 312.94 \\
$\mathrm{HCO^+}$ & 1120.478 & 4.15$\pm$0.28(-20) & 5.09(-20) &  & 4.06 & 334.24 \\
$\mathrm{N_2H^+}$ & 804.439 & $<$6.72(-21) & 2.89(-21) &  & 3.68 & 221.45 \\
$\mathrm{N_2H^+}$ & 1072.557 & $<$6.90(-21) & 1.75(-21) &  & 3.68 & 221.86 \\
$\mathrm{CH^+}$ & 72.137 & $<$2.16(-17) & 1.06(-20) &  & 21.03 & 18.50 \\
\hline
\end{tabular}

==> DIANAmodels/RECX15.tex <==
\centering\begin{tabular}{rr}
\hline
DIANA standard fit model properties &  \\
\hline
minimum dust temperature [K] & 32.16 \\
maximum dust temperature [K] & 1396.33 \\
mass-mean dust temperature [K] & 85.94 \\
minimum  gas temperature [K] & 43.58 \\
maximum  gas temperature [K] & 26981.59 \\
mass-mean  gas temperature [K] & 115.65 \\
mm-opacity-slope (0.85-1.3)mm & 0.82 \\
cm-opacity-slope (5-10)mm & 1.60 \\
mm-SED-slope (0.85-1.3)mm & 2.51 \\
cm-SED-slope (5-10)mm & 3.55 \\
10$\mathrm{\mu m}$ silicate emission amplitude & 1.42 \\
naked star luminosity [$L_\odot$] & 0.11 \\
bolometric luminosity [$L_\odot$] & 0.17 \\
near IR excess ($\lambda=$2.02-6.72$\mathrm{\mu m}$)
 [$L_\odot$] & 0.02 \\
mid IR excess ($\lambda=$6.72-29.5$\mathrm{\mu m}$)
 [$L_\odot$] & 0.02 \\
far IR excess ($\lambda=$29.5-991.$\mathrm{\mu m}$)
 [$L_\odot$] & 0.01 \\
\hline
\end{tabular}


\vspace{0.5cm}\centering\begin{tabular}{lrccccr}
\hline & & \multicolumn{2}{c}{line flux $[\mathrm{W\,m^{-2}}$]} & \multicolumn{2}{c}{FWHM[$\mathrm{km\,s^{-1}}$]} &  \\
species & $\lambda\,$[$\mathrm{\mu m}]$ & observed & model & observed & model & size[AU] \\
\hline
$\mathrm{CO}$ & 866.963 & 8.25$\pm$0.62(-21) & 5.96(-21) & 14.90$\pm$2.30 & 12.64 & 5.42 \\
$\mathrm{OI}$ & 63.183 & 3.05$\pm$0.32(-17) & 2.62(-17) &  & 13.79 & 5.98 \\
$\mathrm{OI}$ & 0.630 & 6.50$\pm$2.50(-17) & 1.26(-16) & 38.00$\pm$10.00 & 20.79 & 3.41 \\
$\mathrm{o\!-\!H_2}$ & 2.121 & 2.50$\pm$0.10(-18) & 1.71(-19) & 18.00$\pm$1.20 & 66.89 & 1.96 \\
$\mathrm{OI}$ & 145.525 & $<$6.00(-18) & 1.37(-18) &  & 13.23 & 5.55 \\
$\mathrm{CII}$ & 157.740 & $<$9.00(-18) & 1.85(-19) &  & 13.96 & 6.04 \\
$\mathrm{CO}$ & 90.162 & $<$9.60(-18) & 7.26(-19) &  & 19.86 & 3.71 \\
$\mathrm{CO}$ & 79.359 & $<$2.40(-17) & 5.64(-19) &  & 24.96 & 2.28 \\
$\mathrm{CO}$ & 72.842 & $<$8.10(-18) & 4.68(-19) &  & 28.67 & 2.05 \\
$\mathrm{o\!-\!H_2O}$ & 180.488 & $<$5.10(-18) & 9.16(-20) &  & 24.22 & 4.27 \\
$\mathrm{o\!-\!H_2O}$ & 179.526 & $<$5.10(-18) & 1.22(-19) &  & 20.09 & 4.79 \\
$\mathrm{o\!-\!H_2O}$ & 78.742 & $<$3.00(-17) & 1.22(-18) &  & 21.32 & 4.80 \\
$\mathrm{p\!-\!H_2O}$ & 89.988 & $<$9.60(-18) & 6.75(-19) &  & 24.22 & 4.36 \\
\hline
\end{tabular}


==> DIANAmodels/TWHya.tex <==
\centering\begin{tabular}{rr}
\hline
DIANA standard fit model properties &  \\
\hline
minimum dust temperature [K] & 7.24 \\
maximum dust temperature [K] & 1112.40 \\
mass-mean dust temperature [K] & 21.05 \\
minimum  gas temperature [K] & 7.35 \\
maximum  gas temperature [K] & 40000.00 \\
mass-mean  gas temperature [K] & 21.29 \\
mm-opacity-slope (0.85-1.3)mm & 1.22 \\
cm-opacity-slope (5-10)mm & 1.39 \\
mm-SED-slope (0.85-1.3)mm & 2.15 \\
cm-SED-slope (5-10)mm & 3.03 \\
10$\mathrm{\mu m}$ silicate emission amplitude & 2.18 \\
naked star luminosity [$L_\odot$] & 0.27 \\
bolometric luminosity [$L_\odot$] & 0.35 \\
near IR excess ($\lambda=$2.02-6.99$\mathrm{\mu m}$)
 [$L_\odot$] & 0.01 \\
mid IR excess ($\lambda=$6.99-29.4$\mathrm{\mu m}$)
 [$L_\odot$] & 0.03 \\
far IR excess ($\lambda=$29.4-972.$\mathrm{\mu m}$)
 [$L_\odot$] & 0.04 \\
\hline
\end{tabular}


\vspace{0.5cm}\centering\begin{tabular}{lrccccr}
\hline & & \multicolumn{2}{c}{line flux $[\mathrm{W\,m^{-2}}$]} & \multicolumn{2}{c}{FWHM[$\mathrm{km\,s^{-1}}$]} &  \\
species & $\lambda\,$[$\mathrm{\mu m}]$ & observed & model & observed & model & size[AU] \\
\hline
$\mathrm{OI}$ & 63.183 & 3.70$\pm$0.10(-17) & 1.38(-16) &  & 1.33 & 97.58 \\
$\mathrm{OI}$ & 145.525 & $<$3.60(-18) & 2.89(-18) &  & 1.46 & 99.53 \\
$\mathrm{CII}$ & 157.740 & $<$3.60(-18) & 2.45(-18) &  & 1.01 & 159.81 \\
$\mathrm{o\!-\!H_2O}$ & 20.341 & 5.20$\pm$2.00(-18) & 1.82(-17) &  & 11.33 & 0.78 \\
$\mathrm{o\!-\!H_2O}$ & 23.859 & 1.10$\pm$0.20(-17) & 2.57(-17) &  & 10.15 & 2.11 \\
$\mathrm{o\!-\!H_2O}$ & 25.365 & 6.60$\pm$2.00(-18) & 2.68(-17) &  & 9.82 & 3.48 \\
$\mathrm{o\!-\!H_2O}$ & 30.525 & 2.40$\pm$0.20(-17) & 2.48(-17) &  & 9.00 & 4.71 \\
$\mathrm{o\!-\!H_2O}$ & 30.870 & 1.60$\pm$0.20(-17) & 2.07(-17) &  & 9.22 & 4.57 \\
$\mathrm{OH_H}$ & 27.393 & 1.50$\pm$0.20(-17) & 2.58(-18) &  & 12.33 & 0.78 \\
$\mathrm{OH_H}$ & 30.277 & 1.55$\pm$0.20(-17) & 2.43(-18) &  & 12.04 & 0.83 \\
$\mathrm{OH_H}$ & 33.875 & 2.90$\pm$0.20(-17) & 2.05(-18) &  & 11.79 & 0.91 \\
$\mathrm{o\!-\!H_2O}$ & 63.323 & $<$7.20(-18) & 5.33(-18) &  & 6.67 & 15.27 \\
$\mathrm{o\!-\!H_2O}$ & 71.946 & $<$6.30(-18) & 4.59(-18) &  & 3.44 & 26.73 \\
$\mathrm{o\!-\!H_2O}$ & 78.742 & $<$6.00(-18) & 5.42(-18) &  & 2.12 & 43.27 \\
$\mathrm{p\!-\!H_2O}$ & 89.988 & 3.10$\pm$0.90(-18) & 3.38(-18) &  & 2.11 & 46.75 \\
$\mathrm{o\!-\!H_2O}$ & 179.526 & $<$7.80(-18) & 3.01(-18) &  & 1.48 & 65.32 \\
$\mathrm{o\!-\!H_2O}$ & 180.488 & $<$8.40(-18) & 6.09(-19) &  & 2.01 & 44.10 \\
$\mathrm{p\!-\!H_2O}$ & 269.272 & 6.10$\pm$0.38(-19) & 1.25(-18) &  & 1.27 & 95.26 \\
$\mathrm{o\!-\!H_2O}$ & 538.288 & 1.70$\pm$0.40(-19) & 2.50(-19) &  & 1.14 & 105.13 \\
$\mathrm{CO}$ & 1300.403 & 1.10$\pm$0.10(-19) & 1.66(-19) &  & 0.82 & 162.40 \\
$\mathrm{CO}$ & 866.963 & 3.92$\pm$0.17(-19) & 5.72(-19) & 0.73$\pm$0.05 & 0.81 & 173.05 \\
$\mathrm{CO}$ & 650.251 & 5.90$\pm$0.60(-19) & 1.26(-18) &  & 0.83 & 164.21 \\
$\mathrm{CO}$ & 433.556 & 6.10$\pm$0.60(-19) & 3.03(-18) &  & 0.91 & 150.24 \\
$\mathrm{CO}$ & 260.239 & 2.13$\pm$0.20(-18) & 3.73(-18) &  & 1.19 & 80.43 \\
$\mathrm{CO}$ & 200.272 & 1.07$\pm$0.25(-17) & 1.65(-18) &  & 1.79 & 50.95 \\
$\mathrm{CO}$ & 144.784 & 3.50$\pm$1.20(-18) & 8.67(-19) &  & 4.38 & 7.65 \\
$\mathrm{CO}$ & 113.457 & 4.40$\pm$1.20(-18) & 6.02(-19) &  & 6.56 & 4.47 \\
$\mathrm{^{13}CO}$ & 1360.227 & 2.00$\pm$0.13(-20) & 2.52(-20) &  & 0.97 & 123.79 \\
$\mathrm{^{13}CO}$ & 906.846 & 4.40$\pm$2.70(-20) & 9.47(-20) &  & 0.97 & 119.66 \\
$\mathrm{^{13}CO}$ & 453.497 & 1.81$\pm$0.29(-19) & 3.99(-19) & 1.43$\pm$0.03 & 1.07 & 98.17 \\
$\mathrm{^{13}CO}$ & 272.204 & 3.60$\pm$0.36(-19) & 1.88(-19) &  & 1.51 & 66.14 \\
$\mathrm{C^{18}O}$ & 1365.430 & 5.00$\pm$1.36(-21) & 6.01(-21) &  & 1.06 & 109.73 \\
$\mathrm{HCO^+}$ & 3361.334 & 2.53$\pm$0.42(-21) & 1.21(-21) &  & 0.72 & 175.88 \\
$\mathrm{HCO^+}$ & 1120.478 & 1.15$\pm$0.19(-19) & 6.59(-20) &  & 0.79 & 177.51 \\
$\mathrm{HCO^+}$ & 840.380 & 2.72$\pm$0.11(-19) & 1.25(-19) & 0.65$\pm$0.05 & 0.82 & 177.76 \\
$\mathrm{HCN}$ & 1127.520 & 7.50$\pm$1.50(-20) & 8.44(-20) &  & 0.81 & 170.46 \\
$\mathrm{HCN}$ & 845.663 & 1.05$\pm$0.31(-19) & 1.49(-19) &  & 0.84 & 161.69 \\
$\mathrm{N_2H^+}$ & 1072.557 & 2.05$\pm$0.43(-20) & 6.60(-21) &  & 0.80 & 125.00 \\
$\mathrm{N_2H^+}$ & 804.439 & 5.72$\pm$0.87(-20) & 1.12(-20) &  & 0.81 & 119.19 \\
$\mathrm{HD}$ & 112.053 & 6.30$\pm$0.70(-18) & 4.76(-19) &  & 1.92 & 63.88 \\
$\mathrm{HD}$ & 56.223 & $<$8.10(-18) & 8.15(-20) &  & 3.34 & 75.82 \\
$\mathrm{OH}$ & 55.890 & 2.22$\pm$0.12(-17) & 4.97(-18) &  & 8.24 & 4.53 \\
$\mathrm{OH}$ & 55.950 & 2.71$\pm$0.15(-17) & 5.84(-18) &  & 7.84 & 4.57 \\
\hline
\end{tabular}
\end{table}

\newpage
\addtocounter{table}{-1}

\begin{table}
\caption{(continued)}
\vspace{0.5cm}\centering\begin{tabular}{lrccccr}
\hline & & \multicolumn{2}{c}{line flux $[\mathrm{W\,m^{-2}}$]} & \multicolumn{2}{c}{FWHM[$\mathrm{km\,s^{-1}}$]} &  \\
species & $\lambda\,$[$\mathrm{\mu m}]$ & observed & model & observed & model & size[AU] \\
\hline
$\mathrm{CO}$ & 4.609 & 6.40$\pm$0.23(-18) & 5.57(-18) & 7.16$\pm$0.20 & 12.32 & 4.61 \\
$\mathrm{CO}$ & 4.657 & 3.68$\pm$0.18(-18) & 2.77(-18) & 7.15$\pm$0.27 & 4.87 & 4.80 \\
$\mathrm{CO}$ & 4.682 & 4.11$\pm$0.20(-18) & 3.39(-18) & 7.68$\pm$0.29 & 4.89 & 5.00 \\
$\mathrm{CO}$ & 4.754 & 6.23$\pm$0.13(-18) & 6.46(-18) & 7.11$\pm$0.21 & 11.65 & 4.61 \\
$\mathrm{CO}$ & 4.793 & 7.22$\pm$0.31(-18) & 6.68(-18) & 7.73$\pm$0.26 & 12.62 & 4.60 \\
$\mathrm{CO}$ & 4.966 & 3.90$\pm$1.00(-18) & 3.20(-18) & 18.50$\pm$1.00 & 16.41 & 0.47 \\
$\mathrm{CO}$ & 4.990 & 2.30$\pm$0.70(-18) & 2.75(-18) & 11.80$\pm$1.00 & 16.46 & 0.47 \\
$\mathrm{OI}$ & 0.630 & 1.20$\pm$0.12(-16) & 2.22(-16) & 10.00$\pm$1.00 & 12.17 & 6.25 \\
$\mathrm{OI}$ & 0.557 & 1.70$\pm$0.50(-17) & 4.35(-17) & 10.00$\pm$1.00 & 19.18 & 0.79 \\
$\mathrm{S^+}$ & 0.406 & 4.40$\pm$0.50(-17) & 1.67(-19) &  & 8.72 & 9.29 \\
$\mathrm{Ne^+}$ & 12.814 & 7.00$\pm$0.20(-17) & 3.42(-17) &  & 4.50 & 45.82 \\
$\mathrm{Ne^{++}}$ & 15.554 & 5.00$\pm$2.00(-18) & 1.25(-17) &  & 4.27 & 88.50 \\
$\mathrm{o\!-\!H_2}$ & 17.033 & 1.20$\pm$0.20(-17) & 5.88(-19) &  & 4.75 & 24.89 \\
$\mathrm{p\!-\!H_2}$ & 12.277 & 7.00$\pm$2.00(-18) & 2.40(-19) &  & 5.62 & 40.89 \\
\hline
\end{tabular}

